On displacement of viscous liquid in a system of parallel tubes

An explicitly solvable quasi 1D model of oil displacement is studied. The problem of recovering of the reservoir geometry is solved by means of a fixed point algorithm. The stability of solution is studied in various functional classes.

==> section7.tex <==
\section{On reestablishing the measure given only a part of curve}

As we showed in previous sections, it is possible to reestablish the measure $\mu$ if we know function $G$ and value $\alpha_{max}$. Now we are interested in following --- what can we say about the measure $\mu$ if we know function $G$ only on some subset of the segment $[0, \alpha_{max}]$?

Result presented in this section will show us, that hole measure $\mu$ can't be reestablished from value $\alpha_{max}$ and function $G$ given on a segment $[0, \alpha_0] \varsubsetneq [0, \alpha_{max}]$.

Recalling formulas which define $V_w(\alpha)$ and $V_o(\alpha)$:

\begin{gather*}
V_w(\alpha) = \frac{1 + \kappa}{2\kappa}\int\limits_0^{\alpha} \frac{\alpha^2 - y^2}{y} d\mu(y) \\
V_o(\alpha) = \int\limits_0^\alpha y d\mu(y) + \frac{1}{1 - \kappa} \int\limits_\alpha^\infty (y - \sqrt{y^2 - (1-\kappa^2) \alpha^2}) d\mu(y))
\end{gather*}

it's easy to see that if measures $\mu_1$ and $\mu_2$ are such that for any $A \subset [0, \alpha_0)$ holds $\mu_1(A) = \mu_2(A)$ and:

\begin{gather*}
\int\limits_{\alpha_0}^\infty (y - \sqrt{y^2 - (1-\kappa^2) \alpha^2}) d\mu_1(y)) = \int\limits_{\alpha_0}^\infty (y - \sqrt{y^2 - (1-\kappa^2) \alpha^2}) d\mu_2(y))
\end{gather*}

then for any $\alpha < \alpha_0$ holds

\begin{gather*}
\begin{cases}
V_{w, \mu_1} (\alpha) = V_{w, \mu_2} (\alpha) \\
V_{o, \mu_1} (\alpha) = V_{o, \mu_2} (\alpha)
\end{cases}
\end{gather*}

And functions $G_1$ and $G_2$ coincide at least on $[0, \alpha_0)$.

Building such measures is quite easy. For example, we can take 

\begin{gather*}
\begin{cases}
\mu_1 = \lambda_{[1, \alpha_0]} + \lambda_{[\alpha_0 + 1, \alpha_0 + 2]} \\
\mu_2 = \lambda_{[1, \alpha_0]} + k^2 \cdot \lambda_{[\frac{\alpha_0 + 1}{k}, \frac{\alpha_0 + 2}{k}]}
\end{cases}
\end{gather*}

where $0 < k < 1 + \dfrac{1}{\alpha_0}$ and $\lambda_{[a, b]}$ denotes Lebesgue measure on section $[a, b]$.
